A VLA Census of the Galactic H II Region Population

The Milky Way contains thousands of H II region candidates identified by their characteristic mid-infrared morphology, but lacking detections of ionized gas tracers such as radio continuum or radio recombination line emission. These targets thus remain unconfirmed as H II regions. With only $\sim$2500 confirmed H II regions in the Milky Way, Galactic surveys are deficient by several thousand nebulae when compared to external galaxies with similar star formation rates. Using sensitive 9 GHz radio continuum observations with the Karl G. Jansky Very Large Array (VLA), we explore a sample of H II region candidates in order to set observational limits on the actual total population of Galactic H II regions. We target all infrared-identified "radio quiet" sources from the WISE Catalog of Galactic H II regions between $245^{\circ}\geq\ell\geq90^{\circ}$ with infrared diameters less than 80$^{\prime\prime}$. We detect radio continuum emission from 50% of the targeted H II region candidates, providing strong evidence that most of the radio quiet candidates are bona fide HII regions. We measure the peak and integrated radio flux densities and compare the inferred Lyman continuum fluxes using models of OB-stars. We conclude that stars of approximately spectral type B2 and earlier are able to create H II regions with similar infrared and radio continuum morphologies as the more luminous H II regions created by O-stars. From our 50% detection rate of "radio quiet" sources, we set a lower limit of $\sim$7000 for the H II region population of the Galaxy. Thus the vast majority of the Milky Way's H II regions remain to be discovered.

==> figset01/figset01.tex <==
%% You can integrate this mark up directly into your ms.tex file
%% by placing the new commands below before your \begin{document}
%% command and everything that follows within the run of text 
%% where you want the figure set to appear.
%\documentclass[12pt,preprint]{aastex}
 
% FIGSET-MACROS-BEGIN
\renewcommand{\noprint}[1]{}
\renewcommand{\figsetstart}{{\bf Fig. Set} }
\renewcommand{\figsetend}{}
\renewcommand{\figsetgrpstart}{}
\renewcommand{\figsetgrpend}{}
\renewcommand{\figsetnum}[1]{{\bf #1.}}
\renewcommand{\figsettitle}[1]{ {\bf #1} }
\renewcommand{\figsetgrpnum}[1]{\noprint{#1}}
\renewcommand{\figsetgrptitle}[1]{\noprint{#1}}
\renewcommand{\figsetplot}[1]{\noprint{#1}}
\renewcommand{\figsetgrpnote}[1]{\noprint{#1}}
%\newcommand{\microns}{\ensuremath{\,\mu{\rm m}}\xspace}
%\bibliography{ref}
% FIGSET-MACROS-END
 
%\begin{document}

\figsetstart
\renewcommand{\thefigure}{A\arabic{figure}}
\figsetnum{A1}
\label{fig:figSet}
\figsettitle{\textit{WISE} composite images of all 146 radio continuum VLA snapshot observations for previously "radio quiet" candidates are available in the online journal.}

\figsetgrpstart
\figsetgrpnum{1.1}
\figsetgrptitle{Image of G090.919+01.493}
\figsetplot{G090_919.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.2}
\figsetgrptitle{Image of G090.192+01.887}
\figsetplot{G090_192.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.3}
\figsetgrptitle{Image of G090.912+01.599}
\figsetplot{G090_912.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.4}
\figsetgrptitle{Image of G091.467+02.826}
\figsetplot{G091_467.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.5}
\figsetgrptitle{Image of G091.582+01.303}
\figsetplot{G091_582.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.6}
\figsetgrptitle{Image of G091.590+02.742}
\figsetplot{G091_590.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.7}
\figsetgrptitle{Image of G092.658+03.054}
\figsetplot{G092_658.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.8}
\figsetgrptitle{Image of G092.677+03.053}
\figsetplot{G092_677.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.9}
\figsetgrptitle{Image of G092.707+03.072}
\figsetplot{G092_707.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.10}
\figsetgrptitle{Image of G093.015+01.235}
\figsetplot{G093_015.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.11}
\figsetgrptitle{Image of G093.370+02.604}
\figsetplot{G093_370.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.12}
\figsetgrptitle{Image of G094.045+01.746}
\figsetplot{G094_045.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.13}
\figsetgrptitle{Image of G094.474+02.178}
\figsetplot{G094_474.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.14}
\figsetgrptitle{Image of G094.712+01.994}
\figsetplot{G094_712.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.15}
\figsetgrptitle{Image of G095.868+03.990}
\figsetplot{G095_868.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.16}
\figsetgrptitle{Image of G096.076+02.562}
\figsetplot{G096_076.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.17}
\figsetgrptitle{Image of G096.538+01.314}
\figsetplot{G096_538.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.18}
\figsetgrptitle{Image of G096.546+01.358}
\figsetplot{G096_546.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.19}
\figsetgrptitle{Image of G097.105+03.165}
\figsetplot{G097_105.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.20}
\figsetgrptitle{Image of G097.131+03.225}
\figsetplot{G097_131.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.21}
\figsetgrptitle{Image of G097.186+03.768}
\figsetplot{G097_186.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.22}
\figsetgrptitle{Image of G097.240+03.300}
\figsetplot{G097_240.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.23}
\figsetgrptitle{Image of G097.276+03.298}
\figsetplot{G097_276.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.24}
\figsetgrptitle{Image of G097.284+03.179}
\figsetplot{G097_284.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.25}
\figsetgrptitle{Image of G097.325+03.226}
\figsetplot{G097_325.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.26}
\figsetgrptitle{Image of G097.693+01.994}
\figsetplot{G097_693.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.27}
\figsetgrptitle{Image of G097.701+03.821}
\figsetplot{G097_701.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.28}
\figsetgrptitle{Image of G097.704+02.048}
\figsetplot{G097_704.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.29}
\figsetgrptitle{Image of G097.786+01.373}
\figsetplot{G097_786.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.30}
\figsetgrptitle{Image of G097.802+01.350}
\figsetplot{G097_802.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.31}
\figsetgrptitle{Image of G097.974+01.494}
\figsetplot{G097_974.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.32}
\figsetgrptitle{Image of G098.908+02.716}
\figsetplot{G098_908.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.33}
\figsetgrptitle{Image of G100.161+01.766}
\figsetplot{G100_161.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.34}
\figsetgrptitle{Image of G100.168+02.082}
\figsetplot{G100_168.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.35}
\figsetgrptitle{Image of G100.213+01.883}
\figsetplot{G100_213.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.36}
\figsetgrptitle{Image of G100.338+01.691}
\figsetplot{G100_338.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.37}
\figsetgrptitle{Image of G102.311+03.677}
\figsetplot{G102_311.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.38}
\figsetgrptitle{Image of G102.334+03.608}
\figsetplot{G102_334.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.39}
\figsetgrptitle{Image of G103.483+01.998}
\figsetplot{G103_483.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.40}
\figsetgrptitle{Image of G103.640+01.087}
\figsetplot{G103_640.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.41}
\figsetgrptitle{Image of G103.690+00.434}
\figsetplot{G103_690.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.42}
\figsetgrptitle{Image of G103.745+02.182}
\figsetplot{G103_745.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.43}
\figsetgrptitle{Image of G103.954+01.097}
\figsetplot{G103_954.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.44}
\figsetgrptitle{Image of G105.433+09.949}
\figsetplot{G105_433.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.45}
\figsetgrptitle{Image of G105.692+00.420}
\figsetplot{G105_962.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.46}
\figsetgrptitle{Image of G106.142+00.129}
\figsetplot{G106_142.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.47}
\figsetgrptitle{Image of G107.156-00.988}
\figsetplot{G107_156.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.48}
\figsetgrptitle{Image of G107.298+05.638}
\figsetplot{G107_298.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.49}
\figsetgrptitle{Image of G108.394-01.046}
\figsetplot{G108_394.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.50}
\figsetgrptitle{Image of G110.054-00.107}
\figsetplot{G110_054.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.51}
\figsetgrptitle{Image of G110.094-00.064}
\figsetplot{G110_094.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.52}
\figsetgrptitle{Image of G110.160+00.040}
\figsetplot{G110_160.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.53}
\figsetgrptitle{Image of G110.812-00.799}
\figsetplot{G110_812.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.54}
\figsetgrptitle{Image of G111.046+01.085}
\figsetplot{G111_046.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.55}
\figsetgrptitle{Image of G111.567+00.751}
\figsetplot{G111_567.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.56}
\figsetgrptitle{Image of G111.774+00.689}
\figsetplot{G111_774.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.57}
\figsetgrptitle{Image of G111.860+00.800}
\figsetplot{G111_860.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.58}
\figsetgrptitle{Image of G111.870+00.881}
\figsetplot{G111_870.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.59}
\figsetgrptitle{Image of G111.941+00.677}
\figsetplot{G111_941.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.60}
\figsetgrptitle{Image of G113.566-00.698}
\figsetplot{G113_566.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.61}
\figsetgrptitle{Image of G113.567-00.657}
\figsetplot{G113_569.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.62}
\figsetgrptitle{Image of G114.569+00.290}
\figsetplot{G114_569.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.63}
\figsetgrptitle{Image of G116.719+03.536}
\figsetplot{G116_719.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.64}
\figsetgrptitle{Image of G119.844+01.518}
\figsetplot{G119_844.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.65}
\figsetgrptitle{Image of G121.750+02.423}
\figsetplot{G121_750.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.66}
\figsetgrptitle{Image of G121.755+02.640}
\figsetplot{G121_755.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.67}
\figsetgrptitle{Image of G123.809-01.781}
\figsetplot{G123_809.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.68}
\figsetgrptitle{Image of G125.331+02.050}
\figsetplot{G125_331.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.69}
\figsetgrptitle{Image of G125.513+02.033}
\figsetplot{G125_513.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.70}
\figsetgrptitle{Image of G127.916+00.657}
\figsetplot{G127_916.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.71}
\figsetgrptitle{Image of G128.315+01.667}
\figsetplot{G128_315.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.72}
\figsetgrptitle{Image of G128.539+01.497}
\figsetplot{G128_539.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.73}
\figsetgrptitle{Image of G129.101+01.965}
\figsetplot{G129_101.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.74}
\figsetgrptitle{Image of G129.806+01.561}
\figsetplot{G129_806.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.75}
\figsetgrptitle{Image of G129.830+01.549}
\figsetplot{G129_830.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.76}
\figsetgrptitle{Image of G131.343-01.188}
\figsetplot{G131_343.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.77}
\figsetgrptitle{Image of G132.361-01.021}
\figsetplot{G132_361.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.78}
\figsetgrptitle{Image of G132.399-00.575}
\figsetplot{G132_399.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.79}
\figsetgrptitle{Image of G133.733+01.498}
\figsetplot{G133_733.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.80}
\figsetgrptitle{Image of G136.348+00.823}
\figsetplot{G136_348.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.81}
\figsetgrptitle{Image of G143.611-01.410}
\figsetplot{G143_611.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.82}
\figsetgrptitle{Image of G145.573+04.336}
\figsetplot{G145_573.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.83}
\figsetgrptitle{Image of G145.583+04.347}
\figsetplot{G145_583.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.84}
\figsetgrptitle{Image of G147.832+00.694}
\figsetplot{G147_832.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.85}
\figsetgrptitle{Image of G148.225+02.241}
\figsetplot{G148_225.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.86}
\figsetgrptitle{Image of G148.449+00.160}
\figsetplot{G148_449.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.87}
\figsetgrptitle{Image of G148.533+01.952}
\figsetplot{G148_533.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.88}
\figsetgrptitle{Image of G148.566+02.162}
\figsetplot{G148_566.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.89}
\figsetgrptitle{Image of G148.809+02.073}
\figsetplot{G148_809.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.90}
\figsetgrptitle{Image of G151.633-00.431}
\figsetplot{G151_633.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.91}
\figsetgrptitle{Image of G155.503+02.640}
\figsetplot{G155_503.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.92}
\figsetgrptitle{Image of G160.104+00.968}
\figsetplot{G160_104.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.93}
\figsetgrptitle{Image of G163.899+04.748}
\figsetplot{G163_899.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.94}
\figsetgrptitle{Image of G164.069+00.436}
\figsetplot{G164_069.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.95}
\figsetgrptitle{Image of G169.936-00.589}
\figsetplot{G169_936.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.96}
\figsetgrptitle{Image of G169.951-00.587}
\figsetplot{G169_951.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.97}
\figsetgrptitle{Image of G170.204+01.990}
\figsetplot{G170_204.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.98}
\figsetgrptitle{Image of G170.830+00.009}
\figsetplot{G170_830.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.99}
\figsetgrptitle{Image of G171.602+00.563}
\figsetplot{G171_602.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.100}
\figsetgrptitle{Image of G171.692+00.564}
\figsetplot{G171_692.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.101}
\figsetgrptitle{Image of G173.328+02.754}
\figsetplot{G173_328.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.102}
\figsetgrptitle{Image of G173.418+02.760}
\figsetplot{G173_418.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.103}
\figsetgrptitle{Image of G173.482+02.445}
\figsetplot{G173_482.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.104}
\figsetgrptitle{Image of G173.485+02.430}
\figsetplot{G173_485.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.105}
\figsetgrptitle{Image of G173.583+02.444}
\figsetplot{G173_583.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.106}
\figsetgrptitle{Image of G173.722+02.693}
\figsetplot{G173_722.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.107}
\figsetgrptitle{Image of G173.779+02.683}
\figsetplot{G173_779.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.108}
\figsetgrptitle{Image of G174.376-00.363}
\figsetplot{G174_376.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.109}
\figsetgrptitle{Image of G174.384-00.371}
\figsetplot{G174_384.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.110}
\figsetgrptitle{Image of G176.462-01.674}
\figsetplot{G176_462.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.111}
\figsetgrptitle{Image of G176.475-01.685}
\figsetplot{G176_475.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.112}
\figsetgrptitle{Image of G181.101+04.223}
\figsetplot{G181_101.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.113}
\figsetgrptitle{Image of G189.032+00.809}
\figsetplot{G189_032.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.114}
\figsetgrptitle{Image of G189.684+00.715}
\figsetplot{G189_684.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.115}
\figsetgrptitle{Image of G192.601-00.048}
\figsetplot{G192_601.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.116}
\figsetgrptitle{Image of G192.617-00.067}
\figsetplot{G192_617.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.117}
\figsetgrptitle{Image of G192.908-00.627}
\figsetplot{G192_908.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.118}
\figsetgrptitle{Image of G194.935-01.222}
\figsetplot{G194_935.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.119}
\figsetgrptitle{Image of G195.666-00.043}
\figsetplot{G195_666.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.120}
\figsetgrptitle{Image of G195.699-00.127}
\figsetplot{G195_699.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.121}
\figsetgrptitle{Image of G195.811-00.215}
\figsetplot{G195_811.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.122}
\figsetgrptitle{Image of G195.822-00.566}
\figsetplot{G195_822.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.123}
\figsetgrptitle{Image of G196.178-00.142}
\figsetplot{G196_178.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.124}
\figsetgrptitle{Image of G197.792-02.356}
\figsetplot{G197_792.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.125}
\figsetgrptitle{Image of G203.373+02.040}
\figsetplot{G203_373.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.126}
\figsetgrptitle{Image of G209.208-00.127}
\figsetplot{G209_208.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.127}
\figsetgrptitle{Image of G211.790-01.354}
\figsetplot{G211_790.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.128}
\figsetgrptitle{Image of G211.896-01.203}
\figsetplot{G211_896.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.129}
\figsetgrptitle{Image of G212.270-01.079}
\figsetplot{G212_270.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.130}
\figsetgrptitle{Image of G212.420-01.126}
\figsetplot{G212_420.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.131}
\figsetgrptitle{Image of G214.456-11.026}
\figsetplot{G214_456.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.132}
\figsetgrptitle{Image of G217.254-00.032}
\figsetplot{G217_258.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.133}
\figsetgrptitle{Image of G217.302-00.059}
\figsetplot{G217_302.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.134}
\figsetgrptitle{Image of G217.307-00.042}
\figsetplot{G217_307.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.135}
\figsetgrptitle{Image of G217.657-00.193}
\figsetplot{G217_657.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.136}
\figsetgrptitle{Image of G221.678-01.897}
\figsetplot{G221_678.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.137}
\figsetgrptitle{Image of G229.569+00.154}
\figsetplot{G229_569.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.138}
\figsetgrptitle{Image of G229.598+00.159}
\figsetplot{G229_598.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.139}
\figsetgrptitle{Image of G232.620+00.995}
\figsetplot{G232_620.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.140}
\figsetgrptitle{Image of G233.676-00.186}
\figsetplot{G233_676.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.141}
\figsetgrptitle{Image of G233.727-00.318}
\figsetplot{G233_727.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.142}
\figsetgrptitle{Image of G234.717-00.913}
\figsetplot{G234_717.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.143}
\figsetgrptitle{Image of G234.729-00.752}
\figsetplot{G234_729.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.144}
\figsetgrptitle{Image of G234.732+00.907}
\figsetplot{G234_732.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.145}
\figsetgrptitle{Image of G237.261-01.306}
\figsetplot{G237_261.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{1.146}
\figsetgrptitle{Image of G243.335-00.012}
\figsetplot{G243_335.pdf}
\figsetgrpnote{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\figsetgrpend

\figsetend

\begin{figure}
\figurenum{1}
\plotone{G090_192.pdf}
\caption{Bands W2 (4.6 \microns\/), W3 (12 \microns\/), and W4 (22 \microns\/) are represented by blue, green, and red, respectively. VLA radio continuum contours at X-band in D configuration are overplotted for regions with newly detected continuum emission. Contours are placed at 33\%, 66\%, and 90\% peak radio continuum flux for sources detected in radio continuum. Peak radio continuum intensities are shown in the bottom left of each panel (in $\mu$Jy) for each detected source and infrared sizes are shown by a scale bar. The VLA beam is shown in red in the bottom right of each image. Most integrations were 4 minute snapshots, but 16 minute integrations are available for 21 sources. These 16 minute integrations are indicated by Deep Integration" labels. Each image is 6$^{\prime}$ on a side, and scale bars represent the regions' infrared angular diameters as cataloged in the \textit{WISE} Catalog of Galactic HII Regions \citep{anderson14}. Measured radio diameters are on average half that of infrared diameters. We smoothed radio continuum emission with a 15$^{\prime\prime}$ boxcar filter for display. Since these objects are all exceedingly faint, there are often much brighter targets in the field that are saturated. When there are multiple candidates within one frame, we only report continuum parameters for the central region.}
\end{figure}

%\end{document}
